Pre-nova Observations of T CrB: A view from the CHARA Array

T CrB is a symbiotic recurrent nova consisting of a red giant and white dwarf with recent eruptions in 1866 and 1946 and an anticipated eruption in the mid 2020s. We report CHARA Array observations obtained with MIRC-X (H -band) and MYSTIC (K-band) in 2022-2025. We fit limb darkened disk models constrained with literature limb darkening coefficients to the squared visibilities as only the first visibility lobe is sampled. The average limb darkened diameter of the star across these epochs is $0.70\pm0.04$ mas in H-band and $0.72\pm0.07$ mas in K-band. Adopting a distance of $914^{+24}_{-22}$ pc, the stellar radius is $69\pm5~R_{\odot}$ in H-band and $71\pm8~R_{\odot}$ in K-band. This is consistent with filling a Roche lobe volume radius of $71~R_{\odot}$ inferred from published orbital solutions. These measurements provide a pre-eruption angular diameter and support a Roche lobe filling donor.

==> models.tex <==
\begin{figure*}[!t]
    \gridline{
        \fig{Munari_2022-03-03_final__nog_linld_final.pdf}{0.20\textwidth}{(a) $\phi=0.77$}
        \fig{Munari_2023-05-09_final__nog_linld_final.pdf}{0.20\textwidth}{(b) $\phi=0.67$}
        \fig{Munari_2023-06-04_final__nog_linld_final.pdf}{0.20\textwidth}{(c)$\phi=0.78$}
        \fig{Munari_2023-09-09_final__nog_linld_final.pdf}{0.20\textwidth}{(d) $\phi=0.21$}}
    \gridline{
       \fig{Munari_2024-06-22_final__nog_linld_final.pdf}{0.20\textwidth}{(e) $\phi=0.47$}
        \fig{Munari_2024-06-23_final__nog_linld_final.pdf}{0.20\textwidth}{(f) $\phi=0.48$}
        \fig{Munari_2025-02-26_final__nog_linld_final.pdf}{0.20\textwidth}{(g) $\phi=0.57$}
       \fig{Munari_2025-02-26_sphere_final_linld_final.pdf}{0.20\textwidth}{(h) Sphere}}
    \caption{Images of the simulated stars used in the simulation  described in Section \ref{sec:analysis}. Phase is calculated adding 0.25 from the phase calculated using $T_{0} (\mathrm{HJD}) = 2459978.37 $ \citep{2025munari}. Thus, $\phi=0$ is superior conjunction, when the RG is behind the WD and $\phi=0.5$ is inferior conjunction, when the RG is in front of the WD.}
    \label{fig:simimages}
\end{figure*}
